Class-Balanced Distillation for Long-Tailed Visual Recognition

Real-world imagery is often characterized by a significant imbalance of the number of images per class, leading to long-tailed distributions. An effective and simple approach to long-tailed visual recognition is to learn feature representations and a classifier separately, with instance and class-balanced sampling, respectively. In this work, we introduce a new framework, by making the key observation that a feature representation learned with instance sampling is far from optimal in a long-tailed setting. Our main contribution is a new training method, referred to as Class-Balanced Distillation (CBD), that leverages knowledge distillation to enhance feature representations. CBD allows the feature representation to evolve in the second training stage, guided by the teacher learned in the first stage. The second stage uses class-balanced sampling, in order to focus on under-represented classes. This framework can naturally accommodate the usage of multiple teachers, unlocking the information from an ensemble of models to enhance recognition capabilities. Our experiments show that the proposed technique consistently outperforms the state of the art on long-tailed recognition benchmarks such as ImageNet-LT, iNaturalist17 and iNaturalist18.

==> background.tex <==
\section{Background}
\label{sec:back}

In this section, we first introduce long-tailed recognition and describe recent training and sampling strategies for this problem.
We then briefly describe knowledge distillation and some of its applications in computer vision.

\subsection{Long-Tailed Recognition}
\label{sec:longtail}

Long-tailed recognition is a supervised learning problem where labeled training data is provided, but with one key distinction: a strong imbalance in terms of instances (images) per class in the training set, following a long-tailed distribution.
The goal is to learn robust models that can recognize all classes, regardless of the number of instances in the training set, which makes it a challenging task.
In the following, we formally define the problem.

% %Long-tailed recognition task aims to learn a model to recognize the examples belonging to the training set. 
% Similar to other supervised learning problems, we are given a training set which contains the examples of various classes.
% The training set is imbalanced and follows a long-tailed distribution over the classes.
% This makes it a challenging task.
% Our goal is to learn robust models that can recognize all classes, regardless of the number of examples they have in the training set.
% We will now formally define the problem.

% \andre{We are using several terminologies to denote class images: instances, examples. I will suggest to use instances/images more consistently, maybe removing ``example'' (since ``instance sampling'' terminology is used throughout the paper).}

\head{Problem Formulation.} We are given a set of $n$ instances (images) $X \defn \{x_1, \ldots, x_n\}$. Each image is labeled according to $Y \defn \{y_1, \ldots, y_n\}$ with $y_i \in C$, where $C \defn \{1,\dots,c\}$ is a label set for $c$ classes.
Let $C_j$ denote the subset of instances labeled as class $j$, and $n_j = |C_j|$ its cardinality.
As previously mentioned, the training set follows a long-tailed distribution, \ie, a majority of $\{n_1,\ldots,n_c\}$ are greatly smaller than $\text{max}(\{n_1,\ldots,n_c\})$.
Despite the training set imbalance, at test time the goal is to accurately recognize all classes, \ie, a balanced test set is used (the number of test images for each class is the same).

% \andre{I think it could be important to mention that we intend to recognize each class accurately, ie the test set should be balanced. Added it above.}

% \head{Problem formulation.} We are given a set of $n$ examples (images) $X \defn (x_1, \ldots, x_n)$. Each image is labeled according to $Y \defn (y_1, \ldots, y_n)$ with $y_i \in C$, where $C \defn \{1,\dots,c\}$ is a label set for $c$ classes.
% Let $C_j$ denote the examples labeled as class $j$, and $n_j = |C_j|$ be the number of examples in class $j$.
% As described above the training set follows a long-tailed distribution, \ie, a majority of $\{n_1,\ldots,n_c\}$ are greatly smaller than $\text{max}(\{n_1,\ldots,n_c\})$.

\head{Model.} 
The learned model (typically a convolutional neural network) takes an input image and outputs class confidence scores. 
We denote the model by $\phi\prm{\theta,W}: \cX \rightarrow \real^c$.
It contains two components, corresponding to the learnable parameters $\theta$ and $W$:
1) a \emph{feature extractor}, mapping each instance $x_i$ to a descriptor $\vv_i \in \real^d$, by $\vv_i \defn f\prm{\theta}(x_i)$;
2) a \emph{network classifier}, typically consisting of a fully connected layer which outputs \emph{logits} $\vz_i \in \real^c$, by $\vz_i \defn g\prm{W}(\vv_i)$, denoting class confidence scores.

% \head{Model. } 
% The learned model (typically a CNN) takes an input example and outputs class confidence scores. 
% We denote the model by $\phi\prm{\theta,W}: \cX \rightarrow \real^c$.
% It contains two components corresponding to the learnable parameters $\theta$ and $W$.
% The \emph{feature extractor} maps each example to a $d$-dimensional descriptor, \ie, $\vv_i \defn f\prm{\theta}(x_i)$, where $\vv_i \in \real^d$ corresponds to the descriptor of the $i$-th example $x_i$.
% The \emph{network classifier} typically consists of a fully connected layer, and outputs \emph{logits}, \ie, a $c$-dimensional class confidence vector:
% $\vz_i \defn g\prm{W}(\vv_i)$ where $\vz_i \in \real^c$. \boqing{FYI, added comma after every \ie}

In this work, we model $g\prm{W}$ as a \emph{cosine classifier}~\cite{LZX+18,GK18}, where feature descriptors and classifier weights are $\ell_2$-normalized before the prediction.
This is motivated by previous work which showed benefits of fixing the norms of classifier weights \cite{kang2019decoupling}.
%\andre{TODO: Ahmet, can you choose good references for these previous two sentences? Feel free to edit the sentences as needed. }
The output becomes $\vz_i \defn \gamma \; \overline{W}^T \overline{\vv_i}$, where $\overline{\vv_i}$ corresponds to the $\ell_2$-normalized version of $\vv_i$, $\overline{W}$ the column-wise $\ell_2$-normalized version of $W$, and $\gamma$ is a scaling parameter which is fixed.
For simplicity, we omit the extra notation for $\ell_2$-normalization and refer to ${\vv_i}$ and $W$ as the $\ell_2$-normalized versions for the rest of this paper.

% \andre{added the exact definition of $g_W$ as matrix multiplication above, which was not there.}

% In this work, we use the \emph{cosine classifier}~\cite{} for classification.
% Feature descriptors and classifier weights are $\ell_2$-normalized before the prediction.
% The output becomes $\vz_i \defn g\prm{ \overline{W} }( \overline{\vv_i})$, where $\overline{\vv_i}$ corresponds to the $\ell_2$-normalized version of $\vv_i$, 
% and $\overline{W}$ corresponds to the column-wise $\ell_2$-normalized version of $W$.
% For the sake of simplicity, we omit the  extra notation for $\ell_2$-normalization  and simply refer to ${\vv_i}$ and $W$ as the $\ell_2$-normalized versions for the rest of this paper.

\head{Training.}
Parameters $\theta$ and $W$ are learned during the training stage.
This is typically achieved by minimizing the loss of the model's output over the training set $X$:
\begin{equation}
L( X, Y; \theta, W) \defn \sum_{i=1}^n \ell \left( \sigma(\vz_i), y_i\right),
\label{eq:loss}
\end{equation}
where $\vz_i = \phi\prm{\theta,W}(x_i)$ is the output of the model, $\sigma(.)$ is the softmax activation function, $\ell(.)$ is the cross-entropy loss function.

%andre{and $\gamma$ is a scaling parameter which is fixed}. 

%\andre{TODO(Ahmet): please confirm if it's learnable, please edit as needed}

\head{Sampling.}
In the context of long-tailed problems, different sampling strategies have been used to adjust the data distribution at training time.
We briefly review two sampling methods which are utilized in this work. 
% \andre{shortened this paragraph a bit}

% \head{Sampling.}
% Due to the imbalanced nature of the training set $X$, one might observe under-fitting to tail classes when training the model. 
% Sampling strategies are proposed to overcome this problem and achieve a more balanced data distribution when evaluating~\eqref{eq:loss}.
% We briefly describe two simple sampling methods which we also utilize in this work. 
% The reader may refer to Kang \etal~\cite{kang2019decoupling} for a more complete list of sampling strategies. \andre{is this last sentence needed? Maybe we could remove it}

\textbf{\emph{Instance sampling}} is a simple method where each instance $x_i \in X$ has the same probability of being chosen in the mini-batch.
Instances from head classes are sampled more frequently than those from tail classes due to the long-tailed nature of the dataset, which may lead to underfitting of tail classes.
%\andre{TODO(Ahmet): as before, confirm if underfitting is the right thing to mention here.} 
Formally, let us denote by $p_j$ the probability of sampling an instance from class $j$.
Under instance sampling, $p_j = n_j / n$. 
% \andre{shortened this paragraph a bit}

% \textbf{\emph{Instance sampling}} is the most-straightforward way of sampling for many computer vision tasks. 
% Under this strategy, each example $x_i \in X$ has the same probability of being chosen in the mini-batch when training the network $\phi\prm{\theta,W}$.
% Examples from head classes are sampled more frequently than those from tail classes due to the long-tailed nature of the dataset.
% Formally, let us denote by $p_j$ the probability of sampling an instance from class $j$.
% Under instance sampling, $p_j$ is directly correlated with the number of examples in a given class, \ie $p_j = n_j / n$. 
% As a result, the network training is more biased toward the head classes.
% This typically causes the model to under-fit tail classes.

\textbf{\emph{Class-balanced sampling}} addresses data imbalance by equalizing $p_j$ across classes.
Under this strategy, each class has the same probability of being selected, \ie, $p_j = 1/c$ for all $j = 1, \ldots, c$.
Even though this strategy balances the data distribution, it also reduces the diversity of examples from head classes.
Tail classes are sampled much more frequently compared to head classes.
As a result, the model tends to overfit the tail classes and a sub-optimal performance may be observed.

% \textbf{\emph{Class-balanced sampling}} attempts to address this problem by balancing $p_j$ across classes.
% Under this strategy, each class has the same probability of being selected, \ie, $p_j = 1/c$ for all $j = 1, \ldots, c$.
% Even though this strategy balances the data distribution, it also reduces the diversity of examples sampled from head classes.
% As a result, a sub-optimal performance may still be observed.

\head{Classifier Re-Training.}
Kang~\etal~\cite{kang2019decoupling} show that it is beneficial to decouple the representation and classifier learning for long-tailed recognition.
The authors propose to learn the two components of the model $\phi\prm{\theta,W}$ with different sampling strategies.
The feature extractor $f\prm{\theta}$ is trained with instance sampling.
Then, $f\prm{\theta}$ is frozen and the network classifier $g\prm{W}$ is trained with class-balanced sampling.
The authors argue that the first stage produces more generalizable features, while the second stage learns a less biased classifier.
Their results showed significant improvement in accuracy for long-tailed recognition benchmarks.
In this work, we improve upon this two-stage framework.

% The authors argue that this strategy encompasses the advantages of two different sampling strategies.
% Instance sampling gives rise to more generalizable feature embeddings and class-balanced sampling produces a less-biased classifier.
% Their results show significant improvement in accuracy for many long-tailed recognition benchmarks.

\subsection{Knowledge Distillation} \label{sec:distillation}
Knowledge distillation~\cite{BCN06,HVD15} refers to transferring information from a \emph{teacher model} $\widehat{\phi}\prm{\widehat{\theta},\widehat{W}}$ to a \emph{student model} $\phi\prm{\theta,W}$.
It has been used in a variety of machine learning and computer vision tasks, such as image classification~\cite{HVD15}, object detection~\cite{CCYH+17}, semi-supervised learning~\cite{TV17} and few-shot learning~\cite{DSM19}.
Distillation is typically achieved by encouraging the student model to mimic the output of the teacher model.
The loss objective from Eq.~\eqref{eq:loss} then becomes:
\begin{multline}
L( X, Y; \theta, W) \defn \sum_{i=1}^n (1-\alpha) \cdot \ell\left( \sigma(\vz_i), y_i\right)  \\
  + \alpha \cdot T^2 \cdot \ell \left( \sigma(\vz_i / T), \sigma(\widehat{\vz_i} / T )\right), \label{eq:distill}
\end{multline}
where $\widehat{\vz_i}  = \widehat{\phi}\prm{\widehat{\theta},\widehat{W}}(x_i)$ is the teacher model's output, $T$ is the temperature parameter used for distillation \cite{HVD15}, and $\alpha$ balances the two loss terms.
Setting $T>1$ increases the weight of the smaller logits and encourages the student model to match its output to their values.
%\andre{TODO(Ahmet): note that I added $\gamma$ in the equation. I think it is used for both the classifier and distillation terms, right? Please correct the equation if it's not the case.}

% Knowledge distillation refers to transferring information between different models~\cite{BCN06,HVD15}.
% It has been used in a variety of machine learning and computer vision tasks, such as model compression~\cite{BCN06}, image classification~\cite{HVD15}, object detection~\cite{CCYH+17}, semi-supervised learning~\cite{TV17}, incremental learning~\cite{LH17} and few-shot learning~\cite{DSM19}.

% Let us assume that there exists a model $\widehat{\phi}\prm{\widehat{\theta},\widehat{W}}$, which we refer to as the \emph{teacher model}. The
% teacher model may contain information beneficial to the generalization of the \emph{student} model $\phi\prm{\theta,W}$.
% Distillation transfers information from the \emph{teacher model} to the \emph{student model} during the training.
% This is typically achieved by encouraging the student model to mimic the output of the teacher model.
% The loss objective~\eqref{eq:loss} then becomes
% \begin{multline}
% L( X, Y; \theta, W) \defn \sum_{i=1}^n (1-\alpha) \cdot \ell\left( \sigma(\vz_i), y_i\right)  \\
%   + \alpha \cdot T^2 \cdot \ell \left( \sigma(\vz_i / T), \sigma(\widehat{\vz_i} / T )\right), \label{eq:distill}
% \end{multline}
% where $\widehat{\vz_i}  = \widehat{\phi}\prm{\widehat{\theta},\widehat{W}}$ is the teacher model's output, $T$ is temperature, and $\alpha$ is a coefficient hyper-parameter.
% Setting $T>1$ increases the weight of the smaller logits and encourages the student model to match its output to their values.

% % temporary, only to get variables in latex format for figures:
% $\vv$

% $f\prm{\theta}$

% $g\prm{W}$

==> ext-plots.tex <==
\usepackage{tikzextern}
\usepackage{pgffor}
\newcommand{\extfig}[2]{\tikzsetnextfilename{fig/extern/#1}{#2}}
\newcommand{\extdata}[1]{}


==> imnet_table.tex <==
\begin{center}
\begin{tabular}{l|llll}
\toprule
Method 					& Many-shot & Mid-shot & Few-shot & All\\
\midrule
% \multicolumn{5}{c}{\textbf{\textsc{Existing Work}}}  \\ \midrule
% Instance 				& 65.9 							& 37.5					& 7.7 					& 44.4 \\
% NCM 					& 56.6~\accneg{(-9.3)} 			& 45.3~\accpos{(+7.8)} 	& 28.1~\accpos{(+20.4)} & 47.3~\accpos{(+2.9)} \\
% cRT 					& 61.8~\accneg{(-4.1)} 			& 46.2~\accpos{(+8.7)} 	& 27.4~\accpos{(+19.7)} & 49.6~\accpos{(+5.2)} \\
% LWS 					& 60.2~\accneg{(-5.7)} 			& 47.2~\accpos{(+9.7)} 	& 30.3~\accpos{(+22.6)} & 49.9~\accpos{(+5.5)} \\
% \midrule
\multicolumn{5}{c}{\textbf{\textsc{Baselines}}}  \\ \midrule
Instance-Cos 			& 67.1 							& 41.6 					& 14.6 						& 47.7  \\
NCM-Cos					& 62.1~\accneg{(-5.0)}			& 46.2~\accpos{(+4.6)}	& 27.2~\accpos{(+12.6)}		& 49.7~\accpos{(+2.0)} \\	
cRT-Cos					& 65.0~\accneg{(-2.1)} 			& 46.8~\accpos{(+5.2)} 	& 25.1~\accpos{(+10.5)} 	& 50.9~\accpos{(+3.2)} \\
\midrule
\multicolumn{5}{c}{\textbf{\textsc{Ours}}}  \\ \midrule
\CBD 					& 69.3~\accpos{(+2.2)} 			& 46.8~\accpos{(+5.2)} 				& 20.2~\accpos{(+5.6)} 				& 51.9~\accpos{(+4.2)}		\\
\CBDncm 				& 66.6~\accneg{(-0.5)} 			& 48.5~\accpos{(+6.9)} 				& 28.5~\accpos{(+13.9)} 			& 52.7~\accpos{(+5.0)}		\\
\CBDens 				& \textbf{70.7}~\accpos{(+3.6)} & 48.0~\accpos{(+6.4)} 				& 20.9~\accpos{(+6.3)} 				& 53.0~\accpos{(+5.3)}		\\
\CBDnens 				& 67.3~\accpos{(+0.2)} 			& \textbf{50.4}~\accpos{(+8.8)} 	& \textbf{31.1}~\accpos{(+16.5)} 	& \textbf{54.3}~\accpos{(+6.6)}		\\

\bottomrule
\end{tabular}
\end{center}


==> inat_table.tex <==
\begin{center}
\begin{tabular}{l|llll}
\toprule
Method 					& Many-shot & Mid-shot & Few-shot & All\\
\midrule
% \multicolumn{5}{c}{\textbf{\textsc{Existing Work}}}  \\ \midrule
% % Instance 				& 73.8 							& 65.6 					& 59.5 						& 64.0 \\
% % cRT 					& 00.0 							& 00.0 					& 00.0 						& 00.0 \\
% % LWS 					& 69.8~\accneg{(-4.0)} 			& 68.4~\accpos{(+2.8)} 	& 66.7~\accpos{(+7.2)} 		& 67.9~\accpos{(+3.9)} \\
% Instance 				& \textbf{75.7} 				& 66.9 					& 61.7 						& 65.8 \\
% NCM 					& 61.0~\accneg{(-14.7)}			& 63.5~\accneg{(-3.4)}	& 63.3~\accpos{(+1.6)} 		& 63.1~\accneg{(-2.7)} \\
% cRT 					& 73.2~\accneg{(-2.5)}			& 68.8~\accpos{(+1.9)}	& 66.1~\accpos{(+4.4)}		& 68.2~\accpos{(+2.4)} \\
% LWS 					& 71.0~\accneg{(-4.7)} 			& 69.8~\accpos{(+2.9)} 	& 68.8~\accpos{(+7.1)} 		& 69.5~\accpos{(+3.7)} \\
% \midrule
\multicolumn{5}{c}{\textbf{\textsc{Baselines}}}  \\ \midrule
Instance-Cos 			& 74.5 							& 65.7 					& 58.0 						& 63.6  \\
NCM-Cos					& 69.4~\accneg{(-5.1)}			& 63.2~\accneg{(-2.5)}	& 59.1~\accpos{(+1.1)}		& 62.2~\accneg{(-1.4)}  \\
cRT-Cos					& 72.0~\accneg{(-2.5)} 			& 66.6~\accpos{(+0.9)} 	& 62.6~\accpos{(+4.6)} 		& 65.5~\accpos{(+1.9)} \\
\midrule
\multicolumn{5}{c}{\textbf{\textsc{Ours}}}  \\ \midrule
\CBD 					& 73.0~\accneg{(-1.5)} 				& 69.8~\accpos{(+4.1)} 				& 66.5~\accpos{(+8.5)} 				& 68.8~\accpos{(+5.2)}		\\
\CBDncm 				& 69.6~\accneg{(-4.9)} 				& 66.4~\accpos{(+0.7)} 				& 64.0~\accpos{(+6.0)} 				& 65.8~\accpos{(+2.2)}		\\
\CBDens 				& \textbf{75.5}~\accpos{(+1.0)} 	& \textbf{73.7}~\accpos{(+8.0)} 	& \textbf{69.4}~\accpos{(+11.4)} 	& \textbf{72.2}~\accpos{(+8.6)}		\\
\CBDnens 				& 72.4~\accneg{(-2.1)} 				& 71.5~\accpos{(+5.8)} 				& 68.9~\accpos{(+10.9)} 			& 70.6~\accpos{(+7.0)}		\\

\bottomrule
\end{tabular}
\end{center}


==> no-plots.tex <==
\newcommand{\extfig}[2]{!!!}
\newcommand{\extdata}[1]{}


==> sota_table_inat17.tex <==
\scriptsize	
\begin{center}
\begin{tabular}{l|c|c}
\toprule
 Method 								& ResNet-50				& ResNet-101 		\\
\midrule
										& All					& All				\\
\midrule
% \multicolumn{3}{c}{\textbf{\textsc{Previous Work}}}  								\\ 
% \midrule
 CB~\cite{CBLoss}						& 58.1					& 60.9				\\
 Rethinking CB~\cite{Jamal_2020_CVPR}	& 59.4					& -					\\
 Feature Aug.~\cite{chu2020feature} 	& 62.0 					& 65.9 		 		\\
 cRT~\cite{kang2019decoupling} 			& 63.9 					& 65.2 		 		\\
 BBN~\cite{Zhou_2020_CVPR} 				& 65.8 					& - 		 		\\
\midrule
% \multicolumn{3}{c}{\textbf{\textsc{Ours}}}  										\\ \midrule
\textbf{Ours} - \CBD 									& 64.6					& 66.5 				\\
\textbf{Ours} - \CBDens 								& \textbf{69.3}			& \textbf{71.3}  	\\
\bottomrule
\end{tabular}
\end{center}

